Sampling in Dirichlet Process Mixture Models for Clustering Streaming Data

Practical tools for clustering streaming data must be fast enough to handle the arrival rate of the observations. Typically, they also must adapt on the fly to possible lack of stationarity; i.e., the data statistics may be time-dependent due to various forms of drifts, changes in the number of clusters, etc. The Dirichlet Process Mixture Model (DPMM), whose Bayesian nonparametric nature allows it to adapt its complexity to the data, seems a natural choice for the streaming-data case. In its classical formulation, however, the DPMM cannot capture common types of drifts in the data statistics. Moreover, and regardless of that limitation, existing methods for online DPMM inference are too slow to handle rapid data streams. In this work we propose adapting both the DPMM and a known DPMM sampling-based non-streaming inference method for streaming-data clustering. We demonstrate the utility of the proposed method on several challenging settings, where it obtains state-of-the-art results while being on par with other methods in terms of speed.

==> figures/fig_aris.tex <==
\begin{figure*}[h]
    \centering
    \newcommand{\MySpace}{\vspace{-.15cm}}
    \newcommand{\MyHeight}{2.95cm}
    \vspace{-.2cm}
    \subcaptionbox{Gaussian 2D\label{Fig:ARI:Gaussian2d}}[0.32\linewidth]{\includegraphics[height=\MyHeight,trim=0.0cm 0.4cm 0.0cm 0.2cm]{../figures/aris/gaussian2d.pdf}\MySpace}
    \subcaptionbox{CoverType\label{Fig:ARI:CoverType}}[0.32\linewidth]{\includegraphics[height=\MyHeight,trim=0.0cm 0.4cm 0.0cm 0.2cm]{../figures/aris/forest.pdf}\MySpace}
    \subcaptionbox{ImageNet100\label{Fig:ARI:ImageNet100}}[0.32\linewidth]{\includegraphics[height=\MyHeight,trim=0.0cm 0.4cm 0.0cm 0.2cm]{../figures/aris/imagenet.pdf}\MySpace}
    \subcaptionbox{ImageNet1K\label{Fig:ARI:ImageNet1K}}[0.32\linewidth]{\includegraphics[height=\MyHeight,trim=0.0cm 0.4cm 0.0cm 0.2cm]{../figures/aris/imagenet_full.pdf}\MySpace}
    \subcaptionbox{Multinomial\label{Fig:ARI:Multinomial}}[0.32\linewidth]{\includegraphics[height=\MyHeight,trim=0.0cm 0.4cm 0.0cm 0.2cm]{../figures/aris/multinomial.pdf}\MySpace}
    \subcaptionbox{20NewsGroups\label{Fig:ARI:20NewsGroups}}[0.32\linewidth]{\includegraphics[height=\MyHeight,trim=0.0cm 0.4cm 0.0cm 0.2cm]{../figures/aris/newsgroup.pdf}\MySpace}
    \captionsetup{justification=centering, singlelinecheck=false}
    \caption{Box plots of the ARI metric for each of the experiments.
    }
     \label{Fig:aris}
     \vspace*{-0.2cm}
\end{figure*}


==> figures/fig_it_metrics.tex <==
\begin{figure}[t]%[h!]
\centering
  \includegraphics[height=5.5cm,trim=0 0 0 0, clip]{../figures/it_count_metrics.pdf}
  \captionsetup{justification=centering, singlelinecheck=false}
  \caption{Performance as a function of $T$. }
\label{fig:it_count_metric}
\end{figure}



==> figures/fig_mean_rand_params.tex <==
\begin{figure}[t]%[h!]
\centering
  \includegraphics[height=5.0cm,trim=0 0 0 0, clip]{../figures/mean_rand_params.pdf}
  \captionsetup{justification=centering, singlelinecheck=false}
  \caption{Box plot of the mean ARI for 10 runs with randomized parameters.}
\label{fig:mean_rand}
\end{figure}



==> figures/fig_nmis.tex <==
\begin{figure*}[t]
    \centering
    \newcommand{\MySpace}{\vspace{-.15cm}}
    \newcommand{\MyHeight}{2.95cm}
    \newcommand{\HeightTrim}{0.4cm}
    \vspace{-.2cm}
    \subcaptionbox{Gaussian 2D\label{Fig:ARI:Gaussian2d}}[0.32\linewidth]{\includegraphics[height=\MyHeight,trim=0.0cm 0.4cm 0.0cm 0.2cm]{../figures/nmis/gaussian2d.pdf}\MySpace}
    \subcaptionbox{CoverType\label{Fig:ARI:CoverType}}[0.32\linewidth]{\includegraphics[height=\MyHeight,trim=0.0cm 0.4cm 0.0cm 0.2cm]{../figures/nmis/forest.pdf}\MySpace}
    \subcaptionbox{ImageNet100\label{Fig:ARI:ImageNet100}}[0.32\linewidth]{\includegraphics[height=\MyHeight,trim=0.0cm 0.4cm 0.0cm 0.2cm]{../figures/nmis/imagenet.pdf}\MySpace}
    \subcaptionbox{ImageNet1K\label{Fig:ARI:ImageNet1K}}[0.32\linewidth]{\includegraphics[height=\MyHeight,trim=0.0cm 0.4cm 0.0cm 0.2cm]{../figures/nmis/imagenet_full.pdf}\MySpace}
    \subcaptionbox{Multinomial\label{Fig:ARI:Multinomial}}[0.32\linewidth]{\includegraphics[height=\MyHeight,trim=0.0cm 0.4cm 0.0cm 0.2cm]{../figures/nmis/multinomial.pdf}\MySpace}
    \subcaptionbox{20NewsGroups\label{Fig:ARI:20NewsGroups}}[0.32\linewidth]{\includegraphics[height=\MyHeight,trim=0.0cm 0.4cm 0.0cm 0.2cm]{../figures/nmis/newsgroup.pdf}\MySpace}
\captionsetup{justification=centering, singlelinecheck=false}    
\caption{Box plots of the NMI metric for each of the experiments.
    }
     \label{Fig:nmis}
\end{figure*}

==> macros.tex <==
 %--------------------------------------------
% Add a period to the end of an abbreviation unless there's one
% already, then \xspace.
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
% \def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{cf}\onedot} \def\Cf{\emph{Cf}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} 
% \def\wrt{with respect to }  % The extra space at the end means \wrt blah would 
% not end up as ``with respect toblah''. 
 
\def\dof{d.o.f\onedot}
% \def\etal{\emph{et al}\onedot}
\def\etal{\emph{et al}\onedot}
% \def\etal{\emph{et al}\onedot}
%
\def\iid{\emph{i.i.d}\onedot}
% \def\pdf{\emph{p.d.f}\onedot}



\makeatother
%--------------------------------------------------

\newcommand{\FIG}{Fig.~}
\newcommand{\FIGS}{Figs.~}
\newcommand{\EQN}{Eq.~}
% \newcommand{\EQN}{Equation }
\newcommand{\EQNS}{Eqs.~}
% \newcommand{\EQNS}{Equations }

%\newcommand{\SEC}{Sec.~}.  Use \autoref or ~\autoref instead.



% integers
\newcommand{\ZZ}{\ensuremath{\mathbb{Z}}}
\newcommand{\RR}{\ensuremath{\mathbb{R}}}
\newcommand{\Rtwo}{\ensuremath{\RR^2}}
\newcommand{\Rthree}{\ensuremath{\RR^3}}
\newcommand{\Rfive}{\ensuremath{\RR^5}}

\newcommand{\Rsix}{\ensuremath{\RR^6}}

\newcommand{\Rn}{\ensuremath{\RR^n}}
\newcommand{\Rd}{\ensuremath{\RR^d}}
\newcommand{\RD}{\ensuremath{\RR^D}}
\newcommand{\Rk}{\ensuremath{\RR^k}}

% 
%positive integers
\newcommand{\Zplus}{\ensuremath{\ZZ^+}}
%positive reals
% \newcommand{\Rplus}{\ensuremath{\RR^+}}

\newcommand{\Rnonneg}{\ensuremath{\RR_{\ge0}}}
\newcommand{\Rpos}{\ensuremath{\RR_{>0}}}


% set notation
% \newcommand{\set}[1]{\ensuremath{{\left\{#1\right\}}}}
\newcommand{\set}[1]{\ensuremath{{\{#1\}}}}
\newcommand{\tuple}[1]{\ensuremath{{(#1)}}}
\newcommand{\tupleLarge}[1]{\ensuremath{{\left(#1\right)}}}
\newcommand{\argmin}[1]{\ensuremath{\operatorname*{arg\,min}_{#1}}}
\newcommand{\argmax}[1]{\ensuremath{\operatorname*{arg\,max}_{#1}}}



\newcommand{\InnerProduct}[2]{\left\langle #1,#2 \right\rangle}

\newcommand{\norm}[1]{{{\left\|#1\right\|}}}
\newcommand{\sign}[1]{{\mathrm{sign}\left(#1\right)}}

\newcommand{\ellTwo}{\ell_2}
\newcommand{\ellTwoNorm}[1]{\norm{#1}_{\ellTwo}}
\newcommand{\ellOne}{\ell_1}




\newcommand{\MATRIX}[2][cccccccccccccccccccc]{\left[
 \begin{array}{#1}
 #2
 \end{array}
\right]}

\newcommand{\Mod}[1]{\ (\mathrm{mod}\ #1)}



% homogeneous coordinates
\newcommand{\bxh}{\widetilde{\bx}}

\newcommand{\RED}[1]{{{\color{red}{#1}}}}  
\newcommand{\BLUE}[1]{{{\color{blue}{#1}}}}
\newcommand{\GREEN}[1]{{{\color{green}{#1}}}}
\definecolor{orcgreen}{RGB}{100,150,100}
\newcommand{\ORCGREEN}[1]{{{\color{orcgreen}{#1}}}}
\newcommand{\MAGENTA}[1]{{{\color{magenta}{#1}}}}  

\definecolor{brown}{RGB}{165,42,42}
\newcommand{\BROWN}[1]{{{\color{brown}{#1}}}}



\newcommand{\REPLACE}[2]{\RED{REPLACE:} \BLUE{#1} \RED{WITH:} \BLUE{#2}}



% In python: print_iterable(['\\bmdefine\\b{0}'.format(x)+'{'+x+'}' for x in 
% string.ascii_letters])

\bmdefine\ba{a}
\bmdefine\bb{b}
\bmdefine\bc{c}
\bmdefine\bd{d}
\bmdefine\be{e}
% \bmdefine\bf{f}  # Clashes with a standard command
\bmdefine\boldf{f}
\bmdefine\bg{g}
\bmdefine\bh{h}
\bmdefine\bi{i}
\bmdefine\bj{j}
\bmdefine\bk{k}
\bmdefine\bl{l}
\bmdefine\bm{m}
\bmdefine\bn{n}
\bmdefine\bo{o}
\bmdefine\bp{p}
\bmdefine\bq{q}
\bmdefine\br{r}
\bmdefine\bs{s}
\bmdefine\bt{t}
\bmdefine\bu{u}
\bmdefine\bv{v}
\bmdefine\bw{w}
\bmdefine\bx{x}
\bmdefine\by{y}
\bmdefine\bz{z}
\bmdefine\bA{A}
\bmdefine\bB{B}
\bmdefine\bC{C}
\bmdefine\bD{D}
\bmdefine\bE{E}
\bmdefine\bF{F}
\bmdefine\bG{G}
\bmdefine\bH{H}
\bmdefine\bI{I}
\bmdefine\bJ{J}
\bmdefine\bK{K}
\bmdefine\bL{L}
\bmdefine\bM{M}
\bmdefine\bN{N}
\bmdefine\bO{O}
\bmdefine\bP{P}
\bmdefine\bQ{Q}
\bmdefine\bR{R}
\bmdefine\bS{S}
\bmdefine\bT{T}
\bmdefine\bU{U}
\bmdefine\bV{V}
\bmdefine\bW{W}
\bmdefine\bX{X}
\bmdefine\bY{Y}
\bmdefine\bZ{Z}


\bmdefine\balpha{\alpha}
\bmdefine\bbeta{\beta}
\bmdefine\bgamma{\gamma}

\bmdefine\bdelta{\delta}
\bmdefine\btheta{\theta}
\bmdefine\blambda{\lambda}
\bmdefine\bphi{\phi}
\bmdefine\bxi{\xi}
\bmdefine\bzeta{\zeta}
\bmdefine\boldeta{\eta}
\bmdefine\bpi{\pi}

\bmdefine\bmu{\mu}
\bmdefine\brho{\rho}
\bmdefine\bomega{\omega}
\bmdefine\bOmega{\Omega}
\bmdefine\bPi{\Pi}

\bmdefine\bvarepsilon{\varepsilon}
\bmdefine\bepsilon{\epsilon}


\bmdefine\bDelta{\Delta}

\bmdefine\bTheta{\Theta}

\bmdefine\bsigma{\sigma}
\bmdefine\bSigma{\Sigma}
\bmdefine\bPsi{\Psi}
\bmdefine\bLambda{\Lambda}



\bmdefine\bzero{0}
\bmdefine\bone{1}
\bmdefine\binfty{\infty}

 \newcommand{\indicator}{\mathds{1}}


% In python 
% print_iterable(['\\newcommand{\\'+'{0}cal'.format(x)+'}{\\mathcal{'+x+'}}' 
% for x in string.ascii_uppercase])
\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Tcal}{\mathcal{T}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}


 \newcommand{\DP}{\mathrm{DP}}
 \newcommand{\DIR}{\mathrm{Dir}}
 
 
 % approximate proportional to
\newcommand{\appropto}{\mathrel{\vcenter{
  \offinterlineskip\halign{\hfil$##$\cr
    \propto\cr\noalign{\kern2pt}\sim\cr\noalign{\kern-2pt}}}}}

